White-Box Performance-Influence Models: A Profiling and Learning Approach

Many modern software systems are highly configurable, allowing the user to tune them for performance and more. Current performance modeling approaches aim at finding performance-optimal configurations by building performance models in a black-box manner. While these models provide accurate estimates, they cannot pinpoint causes of observed performance behavior to specific code regions. This does not only hinder system understanding, but it also complicates tracing the influence of configuration options to individual methods. We propose a white-box approach that models configuration-dependent performance behavior at the method level. This allows us to predict the influence of configuration decisions on individual methods, supporting system understanding and performance debugging. The approach consists of two steps: First, we use a coarse-grained profiler and learn performance-influence models for all methods, potentially identifying some methods that are highly configuration- and performance-sensitive, causing inaccurate predictions. Second, we re-measure these methods with a fine-grained profiler and learn more accurate models, at higher cost, though. By means of 9 real-world Java software systems, we demonstrate that our approach can efficiently identify configuration-relevant methods and learn accurate performance-influence models.

==> conclusion.tex <==
\section{Conclusion}

==> results_acc.tex <==
\begin{table}[t]

\caption{Performance-influence model prediction error (mean absolute percentage error). Measurements: Black-box measurements (BB), coarse-grained measurements (WB1) and fine-grained measurements (WB2). Sampling strategies: Feature-wise (fw), Pair-wise (pw) and Plackett-Burman 125 numeric values and level 5 (125/5).}

\begin{tabular}{llrr}
\toprule
Subject System & Measurements & \multicolumn{2}{c}{Results} \\
 &  &  fw 125/5 & pw 125/5 \\
\midrule
catena & BB &      1.30 &     1.30 \\
        & WB1 &   1072.20 & 25816.00 \\
        & WB2 &      2.50 &     3.50 \\
        \midrule
cpd & BB &      7.89 &     8.74 \\
        & WB1 &    62.29 &    55.57 \\
        & WB2 &     4.64 &    4.83 \\
        \midrule
dc & BB &      9.60 &    52.10 \\
        & WB1 &    762.10 &   857.50 \\
        & WB2 &     11.40 &    11.40 \\
        \midrule
h2 & BB &     51.50 &    52.30 \\
        & WB1 &    550.30 &   966.90 \\
        & WB2 &     10.50 &     9.60 \\
        \midrule
pmd & BB &     27.20 &    19.60 \\
        & WB1 &   1033.80 &  1131.00 \\
        & WB2 &     13.90 &    14.00 \\
        \midrule
pv & BB &      5.60 &    11.70 \\
        & WB1 &   7044.00 &  2736.90 \\
        & WB2 &      5.60 &     5.40 \\
        \midrule
sunflow & BB &     39.20 &        - \\
        & WB1 &  57748.00 &        - \\
        & WB2 &      1.70 &        - \\
\bottomrule
\end{tabular}

    \label{tab:software_systems:results}
\end{table}

==> systems_methods.tex <==
\begin{table}[t]

\caption{Comparing identified hot-spot methods of the subject systems. |$M$| denotes the total number of methods, |$M_\mathit{excl}$| the number of methods excluded from being measured again, and |$M_\mathit{hard}$| the number of filtered methods.}

\addtolength{\tabcolsep}{-3pt}
\begin{tabular}{lrrr}
\toprule
    Subject system &        |$M$| &  |$M_\mathit{excl}$| & |$M_\mathit{hard}$| \\
\midrule
   \textsc{Catena} &         88 &  20  &  7  \\
      \textsc{cpd} &        125 &  9   &  11 \\
       \textsc{dc} &        185 &  17  &  3  \\
       \textsc{H2} &        238 &  12  &  43 \\
      \textsc{pmd} &        218 &  8   &  5  \\
\textsc{Prevayler} &        166 &  22  &  7  \\
  \textsc{Sunflow} &        128 &  7   &  6  \\  
\bottomrule
\end{tabular}

    \label{tab:hot-spots}
\end{table}


==> systems_tracing_info.tex <==
\begin{table}[t]

\caption{Method-specific white-box information. Speedup denotes the factor between the slowest and the fastest configuration of a method; |$F_s$| demotes the number of influential features and interactions system-wide and |$F_\mathit{wb}$| for the method-level; $Frac$ denotes the fraction of the method on the total execution time.}

\addtolength{\tabcolsep}{-3pt}
\begin{tabular}{p{1cm}lll|p{1cm}p{1cm}|lp{1cm}}
\toprule
    Subject system & Speedup & |$F_s$|/|$F_\mathit{wb}$| & $Frac$ & Exact Feature & Method Composition & Varying & High Variation \\
\midrule
    \textsc{Batik} & 3.7 & 4/7& 0.15 & 2 & 20 & 18 & 5 \\
   \textsc{Catena} & $7.6 \cdot 10^5$  & 5/6 & 0.34 & 1 & 24 & 53 & 4 \\
      \textsc{cpd} & 1.5  & 15/1 & 0.02 & 4 & 30 & 86 & 7\\
       \textsc{dc} & $5.9 \cdot 10^3$ & 2/4 & 0.12 & 39 & 70 & 61 & 17 \\
       \textsc{H2} & 2.1  & 3/5 & 0.04 & 5 & 32 & 56 & 3 \\
    \textsc{Kanzi} & 12.4 & 6/3 & 0.09 & 8 & 29 & 116 & 8 \\
      \textsc{pmd} & 4.0  & 4/2 & 0.02 & 28 & 41 & 68 & 15 \\
\textsc{Prevayler} & 25.3 & 2/2 & 0.08 & 7 & 33 & 63 & 4 \\
  \textsc{Sunflow} & 23.3 & 5/3 & 0.15 & 10 & 21 & 29 & 1 \\  
\bottomrule
\end{tabular}

    \label{tab:featuretracing}
\end{table}



\begin{comment}
\begin{table}[t]

\caption{Method-specific white-box information. Speedup denotes the factor between the slowest and the fastest configuration of a method; |$F_s$| demotes the number of influential features and interactions system-wide and |$F_\mathit{wb}$| for the method; $Frac$ denotes the fraction of the method on the total execution time.}

\addtolength{\tabcolsep}{-3pt}
\begin{tabular}{lrrrrrr}
\toprule
    Subject system & Method & Speedup & |$F_s$|/|$F_\mathit{wb}$| & $Frac$ & &  \\
\midrule
    \textsc{Batik} & & & & & &\\
   \textsc{Catena} & G & $7.6 \cdot 10^5$  & 5/6 & 34.2 & 1 & 24\\
      \textsc{cpd} & processCPDSupp.. & 1.5 & 15/1 & 2.4 & &\\
       \textsc{dc} & verticalFromWo.. & $5.9 \cdot 10^3$ & 2/4 & 12.4 & &\\
       \textsc{H2} & getConnection & 2.1 & 3/5 & 4.4 & &\\
    \textsc{Kanzi} &  &  &  &  & &\\
      \textsc{pmd} & visit & 4.0 & 4/2 & 2.1 & &\\
\textsc{Prevayler} & readLine & 25.3 & 2/2 & 0.8 & &\\
  \textsc{Sunflow} & intersect & 23.3 & 5/3 & 15.8 & &\\  
\bottomrule
\end{tabular}

    \label{tab:featuretracing}
\end{table}
\end{comment}

==> t_hist_filter_influences.tex <==
\begin{table}[t]

\caption{Overview of method-call distribution. Cauchy distributed methods are shown with yellow background.}
\begin{tabular}{lrrrr}
\toprule
    % \specialcell{CG vs FG}
    system & method & mean 1-5 & median 1-5 & cv 1-5 \\
\midrule
            Catena &         0.94 &   0.92 \\
               cpd &         0.76 &   0.57 \\
                dc &         0.95 &   0.95 \\
                H2 &         - &   - \\
               pmd &         - &   - \\
         prevayler &         0.99 &   0.88 \\
           Sunflow &         0.93 &   - \\
\bottomrule
\end{tabular}

    \label{tab:context_var_res}
\end{table}

==> t_overhead.tex <==
\begin{table}[t]

\caption{Configuartion-wise linear corellation (LC) and rank corellation (RC) of the black-box measurements (BB) with the coarse-grained profiler (CG) and fine-grained profiler (FG). }

\addtolength{\tabcolsep}{-3pt}
\begin{tabular}{lrrrr}
\toprule
    % \specialcell{CG vs FG}
    Subject System & \multicolumn{2}{c}{BB vs. CG} & \multicolumn{2}{c}{BB vs. FG} \\\cmidrule{2-3}\cmidrule{4-5}
    {}             & LC & RC & LC & RC \\
    % FW 125 5
\midrule
            \textsc{Catena} & 0.94 &  0.98 &     0.81 &  0.95 \\
               \textsc{cpd} & 0.25 &  0.55 &     0.57 &  0.76 \\
                \textsc{dc} & 0.51 &  0.91 &     0.53 &  0.96 \\
                \textsc{H2} & 0.32 &  0.42 &     0.12 &  0.34 \\
               \textsc{pmd} & 0.32 &  0.72 &     0.18 &  0.38 \\
         \textsc{Prevayler} & 0.94 &  0.97 &     0.84 &  0.88 \\
           \textsc{Sunflow} & 0.62 &  0.62 &     0.26 &  0.38 \\
\bottomrule
\end{tabular}

    \label{tab:overhead}
\end{table}
